Avgust: Automating Usage-Based Test Generation from Videos of App Executions

Writing and maintaining UI tests for mobile apps is a time-consuming and tedious task. While decades of research have produced automated approaches for UI test generation, these approaches typically focus on testing for crashes or maximizing code coverage. By contrast, recent research has shown that developers prefer usage-based tests, which center around specific uses of app features, to help support activities such as regression testing. Very few existing techniques support the generation of such tests, as doing so requires automating the difficult task of understanding the semantics of UI screens and user inputs. In this paper, we introduce Avgust, which automates key steps of generating usage-based tests. Avgust uses neural models for image understanding to process video recordings of app uses to synthesize an app-agnostic state-machine encoding of those uses. Then, Avgust uses this encoding to synthesize test cases for a new target app. We evaluate Avgust on 374 videos of common uses of 18 popular apps and show that 69% of the tests Avgust generates successfully execute the desired usage, and that Avgust's classifiers outperform the state of the art.

==> appr-overview.tex <==
\section{Placeholder}

\toolname (\textbf{A}pp \textbf{V}ideo-based \textbf{G}eneration of \textbf{US}age \textbf{T}ests) is an automated approach that is capable of assisting developers with the generation of usage-based tests for mobile applications, which uses neural CV and NLP to map videos and tests to a state machine-based IR model. In this section, we provide an overview of \toolname's workflow, and then describe its three main phases in detail.

\begin{figure*}[h]
	\includegraphics[width=
\textwidth]{figs/design-new.pdf}
\vspace{-2em}
\caption{Overview of \toolname's three-phase workflow}
\vspace{-1em}
	\label{fig:design}
\end{figure*}

\subsection{Approach Overview}

\toolname functions as a developer-in-the-loop automated tool that aims to assist in the creation of usage-based tests. Figure~\ref{fig:design} depicts \toolname's workflow which consists of three main phases: (i) the \textit{Video Collection \& Analysis Phase}, (ii) the \textit{IR Model Generation} phase, and (iii) the \textit{Guided Test Scenario Generation} phase. 

During the \textit{Video Collection \& Analysis} phase crowdsourced workers are tasked with collecting videos of depicting app usages. These videos are then analyzed with a fully automated process which involves deconstructing the video into constituent frames, identifying touch-based actions that were performed on the an app's user interface (which builds upon past work in app video analysis~\cite{bernal2020translatingv2s}), and scraping text from the screen using OCR.

Next, in the \textit{IR Model Generation} phase, \toolname assists the developer of an app with labeling screens and individual GUI-components from processed video frames into categories, which \toolname can then use to generate an app-independent IR Model. This is a semi-automated process wherein a developer is presented with a screen and \toolname provides top-k suggestions for the labels that should be applied to both screens an exercised GUI components. These suggestions are made using a combination of visual- and text-based classifiers that operate upon the screenshots and scraped text of the video frames extracted in the prior phase. After the labels have been applied by the developer, \toolname is able to automatically generate the IR Model for the usage, merging it with other similar usages in a shared database. This phase is intended to be a one-time cost, wherein developers contribute their crowdsourced usages to a collective community database for future use.

Finally, in the \textit{Guided Test Scenario Generation} phase, \toolname assists developers by providing top-k recommendations for actions that should be performed on given screens of an (unseen) target app in order to exercise a specified piece of functionality (e.g., adding an item to the shopping cart). This process starts from the initial screen of the app and runs until the specified feature is exercised. This functions similar to IR Model generation phase, but in reverse, where the model is used in conjunction with \toolname's classification techniques to recommend test scenario inputs to developers.




==> bg.tex <==
%!TEX root = main.tex

\section{Background}
\label{sec:bg}

\yuriy{This needs to be restructured. Section~2 needs to be a motivating
example and a high-level illustration of how the approach works on that
motivating example (so a version of current Section~\ref{sec:Motivating
Example}. Section~\ref{sec:bg:related_work} (Related Work) needs to move to
the end of the paper, after the evaluation; otherwise, you lose the reader's
attention before they even get to your approach. Ideally, the terminology
stuff can be greatly shortened and worked into this new Section~2, so it just
gets defined naturally as you describe the high-level approach. If possible,
whatever parts of the terminology are not necessary in this Section~2, it can
be integrated into the Approach (which will be Section~3), again, being
defined naturally, as you go.}

At a high level, our approach automatically generates \emph{usage-based tests}
based on a 
formal model converted from mobile apps' video recordings. Thus, this
section introduces the necessary concepts and notations related to
usage-based tests
and video manipulations, followed by an  overview of the related work in this
area.
%of
%automated test
%generation.

%\kevin{formalizaion such as Automated Reporting of GUI Design Violations for
%Mobile Apps paper. make sure it's clear that our goals are diff from
%traditional testing.}


\subsection{Usage-based Test Terminology}
\label{sec:bg:usage_test}

As discussed earlier, \emph{usage-based} test generation is an under-explored 
research area, and no existing automated testing techniques can generate such
tests
directly.
Given the nascent nature of this area of work, in this subsection we define
relevant terminology to ground the description of our technique. % aiming to
%establish
%the foundation for future work.

A \textbf{Usage} describes the general flow of exercising a particular software
functionality in an \emph{app-independent} way. % such as via natural language
%description.
As such,
multiple apps may share the same usage, despite their differences at the
implementation level.
%\neno{The preceding sentence begs several questions: What is an abstracted
%functionality? What is a generic way? Can you describe concrete app
%functionality in a generic way? What about an abstracted functionality in a
%specific way? How can "an abstracted functionality" of an app represent "a
%group of functionalities" across apps? Since you are defining your domain of
%discourse here, just watch our for your definitions -- they need to be tight
%and every piece must fit together.}
For
example, a usage may describe the functionality of ``providing
necessary user information to sign up'' (we will refer to this usage as
``sign-up usage'' in short).
%\neno{Which of these two (``sign-up usage'' and ``providing...'') is
%``abstracted functionality'' and which is ``generic way''?}
In different apps, this sign-up usage can be realized in various ways depending
on the app's implementation, such as signing up via the user's \texttt{email}
in
one
app, and signing up via the user's \texttt{username} in another app.
Note that our definition of \emph{usage} is different from the
well-known \emph{use
case}
or
\emph{usage scenario} defined previously~\cite{Rosenberg2007usecase,
Ambler2004MarUML} since they are used to describe the \emph{app-specific}
functionalities
tied to
a particular app's implementation. 
\neno{It may be helpful to provide an example of each? I am not sure this is
clear. It may be just me, but then, I could be your typical reviewer...}
\yixue{i agree it's not clear. see if it's better now. the problem is this
``usage'' thing is not a formal definition, and can be open to interpretation
in
some
way like if i sign up and the username is taken, then I re-signup again with a
different username.
Is
it
the same usage as a typical signup usage? I don't think we want to get into
that
discussion
since
usage
is defined in an
informal/flexible way and you can define your usage in whichever way you want,
but here we're only providing this *concept* to generate a test according to
the usage you defined. not sure if the writing is clear tho}

A \textbf{Usage Trace} is a concrete instance of a \emph{usage} realized for a
given app, covering a sequence of \emph{app-specific} steps to exercise the
corresponding usage. A usage trace can be represented in several different
modalities,
including natural language, executable GUI actions, usage scenario diagrams
using UML~\cite{booch2005uml}, or the video recordings of how a user exercises
the usage.
For example, the {``sign-up usage''} mentioned above may be realized in one app
via the following {usage trace}:
\{ click \texttt{create account} button, 
enter \texttt{username}, enter \texttt{password}, click \texttt{sign up} button
\}. 
Note that in the same app, it is possible to have multiple usage traces for the
same usage since different users may exercise the same usage differently.
%\neno{So, is a usage trace the same thing as a use case or usage scenario?}

A \textbf{Usage Model} is a Finite State Machine (FSM) representing a certain
\emph{usage}
based on a set of \emph{usage traces} from one or multiple apps. The purpose of
the usage model is to capture the possible flows of a given usage learned from 
sample app(s), so that it can be used to guide the usage-based test generation 
for another target app. As the usage model can be learned from different apps 
and used to generate tests for unseen apps, it is critical for the usage model 
to be formalized in an \emph{app-independent} way. 
%For example, in \toolname, we define usage model as a domain-specific finite
%state machine (FSM) based on the videos of a set of \emph{usage traces}
%collected
%from different users. 
We will detail our app-independent formalization of the usage model in
Section~\ref{sec:appr};
other formalizations are possible.
%\neno{Since you say that the purpose of this section is to describe the
%terminology used in this paper specifically, is it necessary to divide the
%general definition of a usage model and your specific embodiment (the "For
%example" sentence)? That is the usage model you have chosen. I think it may
%make more sense to introduce it and then say that other models are possible.
%Also, it would justify the claim that it's a formal model (you choose what
%kind
%of model you want; someone else may choose a not-formal model).}

A \textbf{Usage-based Test}\footnote{For simplicity, ``test'' refers
to ``usage-based test'' in the rest of this paper, unless mentioned otherwise.}
was defined recently~\cite{yixue_zhao_fruiter_2020}
as
the UI test that exercises a given functionality in an app, such as
``sign-in'',
``add item to the shopping cart''. 
%\neno{Are the above examples generic or abstracted, or concrete, or something
%else? Since you are introducing these notions, I think it's important to be
%absolutely clear what the reader is looking at in each instance. Come to think
%of it, shouldn't we also define ``functionality''?}
%\yixue{since i'm reusing FrUITeR's definition, I copied from it as-is. I
%don't think we can modify existing definitions right? I updated the text
%and added
%some
%clarifications tho}
A
usage-based test
consists of a sequence of \emph{GUI events}. We reuse this definition from
prior work~\cite{yixue_zhao_fruiter_2020} in
this
paper. However, we define GUI event differently given our focus on
the \emph{vision-only} solution as mentioned earlier. 
%\neno{Do GUI events
%illustrate or *capture* how a user interacts with the app?} 
%how a user
%interacts
%with
%the app. 
A \textbf{GUI Event} is defined as a triple (\emph{\textbf{s}},
\emph{\textbf{w}}
(optional),
\emph{\textbf{a}}) where
(1) \emph{\textbf{s}} is
the
current
{screen} that shows a snapshot of the current app state; 
(2) optionally, \emph{\textbf{w}} is the GUI
{widget} that the user interacts with (if any); and (3) \emph{\textbf{a}} is
the
corresponding
{action} that the user performs, such as \texttt{click} or \texttt{swipe}.
The GUI widget \emph{w} is optional since certain actions are not associated
with
any
GUI
widgets, such as \texttt{swipe}.
%\neno{What if the
%user
%is not interacting with a widget?}
%An example of the GUI
%event triple is shown in Figure~\ref{fig:motivating}. 
%\yixue{a question speaking of Fig 3. Fig 3 (along with a motivating
%example subsection, which is now in S3.1)
%was in this Background section previously and that's why I'm
%referring to it here. But after discussing with Kevin, we don't think
%it's a motivating example, but rather a simplified example to show some
%artifacts
%of Approach. So I moved it to Approach section for now (Section 3.1).}

\begin{figure}[t]
	\includegraphics[width=0.5\textwidth]{figs/touch_example}
	\center
	\caption{\emph{Non-touch} frame and \emph{touch} frame examples extracted from
the shopping app 6pm's video recording}
	\label{fig:touch}
\end{figure}

\subsection{Terminology on Video Manipulation} 
\label{sec:bg:video}

One of the key contributions of \toolname is to operate on video recordings of
mobile apps to provide a common, and easily accessible medium for collecting
and understanding app usages.
We thus introduce the background information on video manipulations below to
facilitate the understanding of our approach.

\textbf{Video Frames} are the succession of still images that a
given video consists of. For example, Figure~\ref{fig:touch} shows 3 (out of
2801) video frames extracted from a 90-second video using a popular video
processing tool FFmpeg~\cite{FFmpeg}.

%\textbf{Touch} is the physical action of a user interacting with the app by
%touching the device screen. It can be visually identified on the app screen
%through
%the
\textbf{Touch Indicator} is a circle indicating the position of the user's
touch on the device screen as the callout in Figure~\ref{fig:touch} shows. Our
approach requires the touch indicator to be visible in the apps' video
recordings, and this feature can be easily enabled in the device
settings before recording the app video~\cite{EnableTouchIndicator}.
The
opacity
of the touch indicator can vary in different video frames as
Figure~\ref{fig:touch} shows. For each touch, the touch indicator is fully
solid
in
the
first
frame it appears, and then it fades from more to less opaque when a
finger is lifted off
the screen~\cite{bernal2020translatingv2s}. 

\textbf{Touch Frames} are the video frames that contain the touch indicator, 
such as frame 84 and frame 96 in Figure~\ref{fig:touch}; while the rest of the
video frames without the touch indicator are \textbf{Non-Touch
Frames}, such as frame 83. 
\textbf{Touch-Frame Group} is a group of
\emph{consecutive
touch
frames} that contain the same touch indicator of different opacity, such as
frames 84--96 that represent the same touch of ``clicking the
menu
button in the top-left corner of the screen''. 


\textbf{Event Frame} is the \emph{first} frame in a touch-frame
group, such as frame 84 in
Figure~\ref{fig:touch}. It captures the GUI event a user performs via the
touch indicator.
We choose the first frame as event frame because the touch indicator is most 
visible as mentioned above. We will detail how we 
leverage the event
frames to construct a formal usage model in Section~\ref{sec:appr}.

%\neno{I found the above discussion a bit confusing. For one thing, you never
%say what a touch indicator is, and you don't define a frame. Also, does the
%touch-frame group consist of *all* of the frames or just some of them? For
%example, in Figure 1, are these just 3 out of 14 frames?}





%\yixue{anything else should be included? maybe related work on the IR part if
%we claim contributions there e.g., ~\cite{Xue2020Julvisual} }


